CLIP-UP: A Simple and Efficient Mixture-of-Experts CLIP Training Recipe with Sparse Upcycling

Mixture-of-Experts (MoE) models are crucial for scaling model capacity while controlling inference costs. While integrating MoE into multimodal models like CLIP improves performance, training these models is notoriously challenging and expensive. We propose CLIP-Upcycling (CLIP-UP), an efficient alternative training strategy that converts a pre-trained dense CLIP model into a sparse MoE architecture. Through extensive experimentation with various settings and auxiliary losses, we demonstrate that CLIP-UP significantly reduces training complexity and cost. Remarkably, our sparse CLIP B/16 model, trained with CLIP-UP, outperforms its dense counterpart by 7.2% and 6.6% on COCO and Flickr30k text-to-image Recall@1 benchmarks respectively. It even surpasses the larger CLIP L/14 model on this task while using only 30% of the inference FLOPs. We further demonstrate the generalizability of our training recipe across different scales, establishing sparse upcycling as a practical and scalable approach for building efficient, high-performance CLIP models.

==> tabels/methodology-compare.tex <==

\begin{table*}[h]
\caption{Comparing performance of different combination of shared versus separated backbone and training from scratch versus sparse upcycling, and the impact of adding LIMOE auxiliary loss. We benchmark the models on ImageNet Zero-shot classification (Accuracy@1 $\times$\%), COCO and Flickr30k Image retrieval (Recall@1 $\times$\%). T2I: Text-to-Image retrieval; I2T: Image-to-Text retrieval. To isolate the impact of the model's inherent performance, we \textbf{bold} the best model in each task without using on the LIMOE auxiliary loss (the rows with gray background).}
\label{tab:methodology-compare}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
% \setlength{\tabcolsep}{3.5 pt}
% \renewcommand{\arraystretch}{0.8}
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\multicolumn{1}{l}{Model}} &\multicolumn{1}{c}{Imagenet} &\multicolumn{2}{c}{COCO} &\multicolumn{2}{c}{Flickr30K} 
& &Accuray@1 &T2I R@1 &I2T R@1 &T2I R@1 &I2T R@1 \\
\midrule
\rowcolor{lightgray} 
Shared & 69.7 &46.7 &65.6 &71.4 &86.3 \rule{0pt}{3ex} \\
\quad+LIMOE Aux. Loss &73.1 &49.7 &69.7 &75.6 &87.9 \rule{0pt}{3ex} \\
\quad $\Delta$ & +3.4 & +3.0 & +4.1 & +4.2 & +1.6 \\
\cdashline{1-6}
\rowcolor{lightgray} 
Shared-UpCycle &75.2 &51.6 &\textbf{72.7} &78.0 &92.0 \rule{0pt}{3ex} \\
\quad+LIMOE Aux. Loss &73.9 &50.9 &70.1 &73.8 &85.5 \rule{0pt}{3ex} \\
\quad $\Delta$ & -1.3 & -0.7 & -2.6 & -4.2 & -6.5 \\
\cdashline{1-6}
\rowcolor{lightgray} 
Separated &74.5 &\textbf{53.1} &70.6 &78.3 &88.2 \rule{0pt}{3ex} \\
\quad+LIMOE Aux. Loss &72.6 &46.4 &62.6 &73.4 &85.2 \rule{0pt}{3ex} \\
\quad $\Delta$ & -2.0 & -6.7 & -8.0 & -4.9 & -3.0 \\
\cdashline{1-6}
\rowcolor{lightgray} 
Separated-UpCycle &\textbf{76.9} &52.1 &71.5 &\textbf{80.9} &\textbf{92.3} \rule{0pt}{3ex} \\
\quad+LIMOE Aux. Loss &75.9 &52.9 &73.5 &81.3 &92.5 \rule{0pt}{3ex} \\
\quad $\Delta$ & -1.0 & +0.8 & +2.0 & +0.4 & +0.2 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table*}
